Data-inspired modeling of accidents in traffic flow networks using the Hawkes process

We consider hyperbolic partial differential equations (PDEs) for a dynamic description of the traffic behavior in road networks. These equations are coupled to a Hawkes process that models traffic accidents taking into account their self-excitation property which means that accidents are more likely in areas in which another accident just occurred. We discuss how both model components interact and influence each other. A data analysis reveals the self-excitation property of accidents and determines further parameters. Numerical simulations using risk measures underline and conclude the discussion of traffic accident effects in our model.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{A Hierarchy of Traffic Accident Models containing the Self-Excitation property}{S. G\"ottlich, T. Schillinger}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A Hierarchy of Traffic Accident Models containing the Self-Excitation property\thanks{Submitted to the editors DATE.
\funding{This work was funded by ??}}}

% Authors: full names plus addresses.
\author{Simone G\"ottlich\thanks{University of Mannheim, Department of Mathematics, 68131 Mannheim, Germany (\email{goettlich@uni-mannheim.de})}
\and Thomas Schillinger\thanks{University of Mannheim, Department of Mathematics, 68131 Mannheim, Germany (\email{schillinger@uni-mannheim.de}}}
%\and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

